AxBench: Steering LLMs? Even Simple Baselines Outperform Sparse Autoencoders

Fine-grained steering of language model outputs is essential for safety and reliability. Prompting and finetuning are widely used to achieve these goals, but interpretability researchers have proposed a variety of representation-based techniques as well, including sparse autoencoders (SAEs), linear artificial tomography, supervised steering vectors, linear probes, and representation finetuning. At present, there is no benchmark for making direct comparisons between these proposals. Therefore, we introduce AxBench, a large-scale benchmark for steering and concept detection, and report experiments on Gemma-2-2B and 9B. For steering, we find that prompting outperforms all existing methods, followed by finetuning. For concept detection, representation-based methods such as difference-in-means, perform the best. On both evaluations, SAEs are not competitive. We introduce a novel weakly-supervised representational method (Rank-1 Representation Finetuning; ReFT-r1), which is competitive on both tasks while providing the interpretability advantages that prompting lacks. Along with AxBench, we train and publicly release SAE-scale feature dictionaries for ReFT-r1 and DiffMean.

==> tables/human_eval.tex <==
\begin{table}[h!]
    \small
    \centering
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Stats} & \textbf{Overall score} & Concept score & Instruct score & Fluency score \\
    \midrule
    \emph{Pearson correlation} & & & & \\
    \quad \texttt{gpt-4o-mini} - Human & & & & \\
    \quad Human - Human & & & & \\
    \quad Random & & & & \\ \midrule
    \emph{Spearman correlation} & & & & \\
    \quad \texttt{gpt-4o-mini} - Human & & & & \\
    \quad Human - Human & & & & \\
    \quad Random & & & & \\ 
    \bottomrule
    \end{tabular}
    \caption{Correlations between scores rated by our LLM judges and human. For the \texttt{gpt-4o-mini} - Human condition, we use averaged human ratings.}
\end{table}
